I Can't Believe It's Not Scene Flow!

Current scene flow methods broadly fail to describe motion on small objects, and current scene flow evaluation protocols hide this failure by averaging over many points, with most drawn larger objects. To fix this evaluation failure, we propose a new evaluation protocol, Bucket Normalized EPE, which is class-aware and speed-normalized, enabling contextualized error comparisons between object types that move at vastly different speeds. To highlight current method failures, we propose a frustratingly simple supervised scene flow baseline, TrackFlow, built by bolting a high-quality pretrained detector (trained using many class rebalancing techniques) onto a simple tracker, that produces state-of-the-art performance on current standard evaluations and large improvements over prior art on our new evaluation. Our results make it clear that all scene flow evaluations must be class and speed aware, and supervised scene flow methods must address point class imbalances. We release the evaluation code publicly at https://github.com/kylevedder/BucketedSceneFlowEval.

==> abstract_old.tex <==
State-of-the-art scene flow methods consistently fail to capture the motion of smaller objects with fewer points (e.g.\ {\tt PEDESTRIANS} and {\tt WHEELED VRUs}). However, existing evaluation metrics fail to characterize this because average error is dominated by large objects (e.g.\ {\tt CAR} and {\tt OTHER VEHICLES}) which are responsible for most moving points. To address this limitation, we propose \emph{\oureval{}}, a new evaluation protocol that measures speed-normalized performance on a per-metaclass basis. Additionally, we present a frustratingly simple supervised scene flow baseline using an off-the-shelf pretrained detector and simple tracker that improves {\tt PEDESTRIANS} dynamic EPE by 20\% \neehar{Replace with exact number}. Our method, \emph{\ourmethod{}}, achieves state-of-the-art performance on standard evaluation protocols, and significantly outperforms prior work by over 10\% \neehar{Replace with exact number} on our improved metric.
